A Dual Formulation for Probabilistic Principal Component Analysis

In this paper, we characterize Probabilistic Principal Component Analysis in Hilbert spaces and demonstrate how the optimal solution admits a representation in dual space. This allows us to develop a generative framework for kernel methods. Furthermore, we show how it englobes Kernel Principal Component Analysis and illustrate its working on a toy and a real dataset.

==> archive/0-abstract.tex <==
\begin{abstract}
In this paper, we give a dual interpretation of the probablistic principal component analysis. We further show how it connects to classical PCA, but also restricted kernel machines or restricted boltzmann machines. We further show how particular metrics between probability distributions introduce a dual representation and study the particular case of the Wasserstein distance.
\end{abstract}

==> archive/1-introduction.tex <==
\section{Introduction}
\label{sec:introduction}

==> archive/2-pca.tex <==
\section{Principal Component Analysis}
\label{sec:pca}


The problem when dealing with kernels is that the feature representation may lie in an infinite dimensional Hilbert space: we therefore must consider linear operators in general instead of matrix operations. For the sake of convenience and following~\cite{convex_pca}, we will therefore use bra-ket notation~\cite{braket}. 


Following~\cite{convex_pca}, we will define 

\subsection{Probabilistic PCA (Primal)}
We define the visible variables as $\bm{v} \in \mathbb{R}^{d}$, the hidden variables as $\bm{h} \in \mathbb{R}^{f}$ and the interconnection operator as $\bm{W} \in \mathbb{R}^{d \times f}$. Following from~\cite{ppca}, we define the prior distribution
\begin{equation}
    \bm{v}|\bm{h},\bm{W} \sim \mathcal{N}\left(\bm{W}\bm{h}, \sigma^2\bm{I}_d\right),
\end{equation}
together with the prior $\bm{h} \sim \mathcal{N}(\bm{0},\bm{I})$, of which we can retrieve the marginal by integrating the joint distribution over the hidden variables
\begin{equation}
    \bm{v}|\bm{W} \sim \mathcal{N}(\bm{0}, \bm{\Sigma}_{\bm{v}|\bm{W}}),
\end{equation}
with $\bm{\Sigma}_{\bm{v}|\bm{W}} = \bm{W}\bm{W}^\top + \sigma^2\bm{I}_d$. The solutions for the interconnection matrix is given by
\begin{equation}
\label{eq:interconnection-ml}
    \bm{W}_{\text{ML}} = \bm{U}_f\left(\frac{\bm{\Lambda}_f^2}{N} - \sigma^2\bm{I}_f\right)^{1/2}\bm{R}^\top,
\end{equation}
with $\bm{R}$ an arbitrary rotation matrix (full rank).

\subsection{Dual Formulation}
Without loss of generality, by the probabilistic representer theorem (check further required), we can assume $\bm{W} = \bm{\Phi}\bm{A}$ with $\bm{\Phi} \in \mathbb{R}^{d \times N}$ and $\bm{A} \in \mathbb{R}^{N \times f}$. To rewrite the marginal of the visible variables as
\begin{equation}
    \label{eq:dual-visible-marginal}
    \bm{v}|\bm{A} \sim \mathcal{N}(\bm{0},\bm{\Sigma}_{\bm{v}|\bm{A}} ),
\end{equation}
with $\bm{\Sigma}_{\bm{v}|\bm{A}} = \bm{\Phi}\bm{A}\bm{A}^\top\bm{\Phi}^\top + \sigma^2\bm{I}_d$.

\subsection{Maximum Likelihood Estimator}
The likelihood of Eq.~\ref{eq:dual-visible-marginal} is given by
\begin{eqnarray}
    \mathcal{L} &=& -\frac{N}{2}\left\{ d\ln(2\pi) + \ln\left|\bm{\Sigma}_{\bm{v}|\bm{A}} \right|  + \frac1N\sum_{i=1}^{N} \bm{v}_i^\top\bm{\Sigma}_{\bm{v}|\bm{A}} ^{-1}\bm{v}_i\right\}, \\
    &=& -\frac{N}{2}\left\{ d\ln(2\pi) + \ln\left|\bm{\Sigma}_{\bm{v}|\bm{A}}\right|  + \frac1N\tr\left(\bm{C}\bm{\Sigma}_{\bm{v}|\bm{A}}^{-1} \right) \right\},
\end{eqnarray}
with (non-weighted) covariance matrix $\bm{C} = \sum_i \bm{v}_i\bm{v}_i^\top = \bm{\Phi}\bm{\Phi}^\top$. We can now look at the evolution of the likelihood in function of $\bm{A}$:
\begin{equation}
    \label{eq:likelihood-dual-derivative}    \frac{\partial\mathcal{L}}{\partial\bm{A}} = N \bm{\Phi}^\top \bm{\Sigma}_{\bm{v}|\bm{A}}^{-1} \bm{\Phi}\bm{A} - \bm{\Phi}^\top \bm{\Sigma}_{\bm{v}|\bm{A}} ^{-1} \bm{\Phi}\bm{\Phi}^\top \bm{\Sigma}_{\bm{v}|\bm{A}} ^{-1} \bm{\Phi}\bm{A} = 0,
\end{equation}
or
\begin{equation}
    N\bm{\Phi}^\top \bm{\Sigma}_{\bm{v}|\bm{A}}^{-1}\bm{\Phi}\bm{A} = \bm{\Phi}^\top \bm{\Sigma}_{\bm{v}|\bm{A}}^{-1}\bm{\Phi}\bm{\Phi}^\top\bm{\Sigma}_{\bm{v}|\bm{A}}^{-1}\bm{\Phi}\bm{A}.
\end{equation}

\subsubsection{Stationary Points}
We first consider the decomposition of $\bm{\Phi} = \bm{U}\bm{\Lambda}\bm{V}^\top$ and notice that $\bm{K} = \bm{\Phi}^\top\bm{\Phi} = \bm{V}\bm{\Lambda}^2\bm{V}^\top$ and $\bm{C} = \bm{\Phi}\bm{\Phi}^ \top = \bm{U}\bm{\Lambda}^2\bm{U}^\top$. We have the relation
\begin{eqnarray}
    \bm{\Phi}^\top \bm{\Sigma}_{\bm{v}|\bm{A}}^{-1}\bm{\Phi} &=& \bm{\Phi}^\top \left(\bm{\Phi}\bm{A}\bm{A}^\top\bm{\Phi}^\top + \sigma^2\bm{I}_d\right)^{-1}\bm{\Phi}, \\
    &=& \bm{V}\bm{\Lambda}\bm{U}^\top\left(\bm{U}\bm{\Lambda}\bm{V}^\top\bm{A}\bm{A}^\top\bm{V}\bm{\Lambda}\bm{U}^\top + \sigma^2\bm{I}_d\right)^{-1}\bm{U}\bm{\Lambda}\bm{V}^\top, \\
    &=& \bm{V}\left(\bm{V}^\top\bm{A}\bm{A}^\top\bm{V} + \sigma^2\bm{\Lambda}^{-2}\right)^{-1} \bm{V}^\top
\end{eqnarray}

As the latter can be assumed of full rank, eq~\ref{eq:likelihood-dual-derivative} now becomes:
\begin{eqnarray}
    N\bm{A} &=& \bm{V}\left(\bm{V}^\top\bm{A}\bm{A}^\top\bm{V} + \sigma^2\bm{\Lambda}^{-2}\right)^{-1} \bm{V}^\top\bm{A},
\end{eqnarray}
We will now assume that $d > N$ (thus $\bm{V}\bm{V}^\top = \bm{I}_N$) and $\bm{A} = \bm{X}\bm{L}\bm{Y}^\top$, with $\bm{X} \in \mathbb{R}^{N \times f}$, $\bm{Y} \in \mathbb{R}^{f \times f}$ and $\bm{L}$ diagonal:
\begin{eqnarray}
    N\bm{X}\bm{L}\bm{Y}^\top &=& \bm{V}\left(\bm{V}^\top\bm{X}\bm{L}\bm{Y}^\top\bm{Y}\bm{L}\bm{X}^\top\bm{V} + \sigma^2\bm{\Lambda}^{-2}\right)^{-1} \bm{V}^\top\bm{X}\bm{L}\bm{Y}^\top, \\
    N\bm{X} &=& \left(\bm{X}\bm{L}^2\bm{X}^\top + \sigma^2\bm{V}\bm{\Lambda}^{-2}\bm{V}^\top \right)^{-1}\bm{X}. 
\end{eqnarray}
We can multiply both sides by $\bm{X}^\top$ (can we?) and get
\begin{eqnarray}
    N\bm{I}_f &=& \bm{X}^\top \left(\bm{X}\bm{L}^2\bm{X}^\top + \sigma^2\bm{K}^{-1}\right)^{-1} \bm{X}, \\
    N\bm{I}_f &=& \left( \bm{L}^2 + \sigma^2\bm{X}^\top\bm{K}^{-1}\bm{X}\right)^{-1}, \\
    \frac{1}{N}\bm{I}_f &=& \bm{L}^2 + \sigma^2\bm{X}^\top\bm{K}^{-1}\bm{X}, \\
    \frac{1}{\sigma^2}\left(\frac{1}{N}\bm{I}_f - \bm{L}^2\right) &=& \bm{X}^\top\bm{K}^{-1}\bm{X}.
\end{eqnarray}
This is an eigenvalue problem. We can thus conclude that $\bm{X}^\top = \bm{V}_f$ and $\bm{L} = \left( \frac{1}{N}\bm{I}_f - \sigma^2\bm{\Lambda}^{-2}\right)^{1/2}$. By consequence,
\begin{equation}
    \bm{A} = \bm{V}_f^\top \left( \frac{1}{N}\bm{I}_f - \sigma^2\bm{\Lambda}^{-2}\right)^{1/2}\bm{Y}^\top.
\end{equation}
We can also verify the consistency with the interconnection operator
\begin{equation}
    \bm{W}_{\text{ML}} = \bm{U}\bm{\Lambda}\bm{V}^\top \bm{V}_f \left( \frac{1}{N}\bm{I}_f - \sigma^2\bm{\Lambda}^{-2}\right)^{1/2}\bm{R}^\top,
\end{equation}
which retrieves eq.~\ref{eq:interconnection-ml} with $\bm{Y}=\bm{R}$.

 \begin{table}[t]
     \centering
     \begin{tabular}{l|p{.12\textwidth}|p{.12\textwidth}|p{.12\textwidth}}
    & $ d < N$ & $d=N$ & $ d > N $ \\ \hline
   $\bm{U}$ (primal) & $\bm{U}^\top\bm{U} = \bm{I}_d$ \newline $\bm{U}\bm{U}^\top = \bm{I}_d$ & $\bm{U}^\top\bm{U} = \bm{I}_d$ \newline $\bm{U}\bm{U}^\top = \bm{I}_d$ & $\bm{U}^\top\bm{U} = \bm{I}_d$ \newline $\bm{U}\bm{U}^\top = \mathbb{P}_d$  \\ \hline
   $\bm{V}$ (dual) & $\bm{V}^\top\bm{V} = \bm{I}_N$ \newline $\bm{V}\bm{V}^\top = \mathbb{P}_N$ & $\bm{V}^\top\bm{V} = \bm{I}_N$ \newline $\bm{V}\bm{V}^\top = \bm{I}_N$  & $\bm{V}^\top\bm{V} = \bm{I}_N$ \newline $\bm{V}\bm{V}^\top = \bm{I}_N$ 
\end{tabular}
     \caption{Projection dimensions ($\mathbb{P}$ indicates a projector approximating the identity).}
     \label{tab:projectors}
 \end{table}

 \subsubsection{Hidden variables}
The posterior distribution for the hidden variables \cite{ppca} is given by
\begin{equation}
    \bm{h} | \bm{v} \sim \mathcal{N}\left(\bm{M}^{-1}\bm{W}\bm{v},\sigma^2\bm{M}^{-1}\right).
\end{equation}
Filling in the maximum likelihood estimator for the interconnection matrix $\bm{W}$ (or equivalently $\bm{A}$), we get $\bm{M}^{-1} = \bm{\Lambda}_f^{-2}/N$. The maximum a posteriori for the hidden variables (using $\bm{W}$ or $\bm{A}$) is by consequence
\begin{eqnarray}
    N\bm{\Lambda}_f^2\bm{h} | \bm{v} &=& \bm{W}^\top\bm{v}, \\
    N\bm{\Lambda}_f^2\bm{h} | \bm{k} &=& \bm{A}^\top\bm{k},
\end{eqnarray}
with $\bm{k} = \bm{v}^\top\left[\bm{v}_1 \ldots \bm{v}_N\right]$.

==> archive/3-rkm.tex <==
\section{Restricted Kernel Machines}
\label{sec:rkm}


The posterior distribution of the hidden variables given the visible ones can be rewritten as
\begin{equation}
    p(\bm{h}|\bm{v}) = \frac{1}{Z}\exp\left(-\frac{1}{2N\sigma^2}\bm{h}^\top\bm{\Lambda}_f^2\bm{h} + \frac{1}{\sigma^2}\bm{v}^\top\bm{W}_{\text{ML}}\bm{h}\right),
\end{equation}
where $\bm{\Lambda}_f^2/N$ are the eigenvectors of the covariance matrix $\sum_i \bm{v}_i\bm{v}_i^\top$.

==> archive/4-wasserstein.tex <==
\section{Wasserstein PCA}
\label{sec:wasserstein}


\subsection{Gaussian Assumption}
An insteresting case happens if we suppose the empirical data to be Gaussian and we decide to minimize the Wasserstein distance instead of the MLE/KL. In the full rank case of $\bm{W}$ with $\sigma^2 = 0$, the model allows the posterior distribution to perfectly match the empirical one, hence retrieving the same answer as for the MLE. Interestingly, this is also the case for $\sigma^2 \neq 0$.

Minizing the wasserstein distance between two gaussians of same mean $\mathcal{N}(\bm{\mu},\bm{\Sigma}_1)$ and $\mathcal{N}(\bm{\mu},\bm{\Sigma}_2)$ amounts to minimize the Bures metric
\begin{equation}
    \mathcal{B}(\bm{\Sigma}_1,\bm{\Sigma}_2) = \tr\left\{ \bm{\Sigma}_1 + \bm{\Sigma}_2 -2\left(\bm{\Sigma}_1^{1/2}\bm{\Sigma}_2\bm{\Sigma}_1^{1/2}\right)^{1/2}\right\}.
\end{equation}

We have from \cite{bhatia2019bures}

\begin{equation}
    \mathcal{B}(\bm{\Sigma}_1,\bm{\Sigma}_2) = \underset{\text{$\bm{R}$ is orthogonal}}{\min}\left\lVert \bm{\Sigma}_1^{1/2} - \bm{\Sigma}_2^{1/2}\bm{R} \right\rVert_2
\end{equation}

We also have, if we suppose $\bm{W} = \bm{X}\bm{L}\bm{Y}^\top$ and as earlier $\bm{\Phi} = \bm{U}\bm{\Lambda}\bm{V}^\top$.
\begin{eqnarray}
    \bm{\Sigma}_1^{1/2} &=& \bm{X}\left(\bm{L}^2 + \sigma^2\bm{I}\right)^{1/2}\bm{X}^\top,\\
    \bm{\Sigma}_2^{1/2} &=& \frac{1}{\sqrt{N}}\bm{U}\bm{\Lambda}\bm{U}^\top.
\end{eqnarray}.

Hence the total optimization problem now amounts to

\begin{equation}
    \bm{W}_{\text{Wass}} = \underset{\substack{\text{$\bm{U}$ orthogonal}\\ \text{$\bm{L}$ diagonal}}}{\mathrm{argmin}} \underset{\text{$\bm{R}$ is orthogonal}}{\min}\left\lVert \bm{X}\left(\bm{L}^2 + \sigma^2\bm{I}\right)^{1/2}\bm{X}^\top - \frac{1}{\sqrt{N}}\bm{U}\bm{\Lambda}\bm{U}^\top\bm{R} \right\rVert_2.
\end{equation}


\subsection{No assumption}

Assuming the distribution of $\bm{v}$, we can sample from it with $\bm{u} \sim \mathcal{N}\left(\bm{\mu},\bm{I}_f\right)$ with
\begin{equation}
    \bm{v} = \bm{\mu} + \bm{P}\bm{u},
\end{equation}
such that $\bm{P}\bm{P}^\top = \bm{W}\bm{W}^\top + \sigma^2$. If $\sigma^2 = 0$, we have trivially $\bm{P} = \bm{W}$. If $\sigma^2 \neq 0$ and $\bm{W}$ is of full rank, we have assuming $\bm{W} = \bm{U}\bm{L}\bm{V}^\top$
\begin{equation}
    \bm{P} = \bm{U}\left(\bm{L}^2 + \sigma^2\bm{I}\right)^{1/2}\bm{U}^\top.
\end{equation}

Considering the dual only in the case $\sigma^2 = 0$, we have $\bm{k} = \bm{\Phi}^\top\bm{v}$. By consequence, we have 
\begin{eqnarray}
    \bm{k} &=& \bm{\Phi}^\top\bm{\mu} + \bm{\Phi}^\top\bm{P}\bm{u}, \\
    &=& \bar{\bm{k}} + \bm{K}\bm{A}\bm{u}.
\end{eqnarray}

\subsection{Optimization}

The minimization of the Wasserstein loss is given by
\begin{equation}
    \nabla \mathcal{L}(\theta) = \left[ \partial x(\theta)\right]^\top \left( \nabla\mathcal{F}(x(\theta))\right),
\end{equation}
with
\begin{equation}
    \nabla \mathcal{F}(\theta) = \left( \sum_{j=1}^M P_{i,j}\nabla_1 c(x_1,y_j)\right)_{i=1}^N
\end{equation}

Given our parameters $\theta = \left\{\bm{W},\bm{\mu}\right\}$, we have

==> archive/5-expe.tex <==
\label{Experiments}
\label{sec:expe}

==> archive/6-conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

==> content/4-rkm.tex <==
\section{Restricted Kernel Machines}
In this section, we present the connections of our primal and dual probabilistic model with \emph{Restricted Kernel Machines} (RKM)~\cite{rkm}. The latter essentially combines the variational approach of \emph{Principal Component Analysis}~\cite{lssvm-pca} with the Fenchel-Young inequality to provide a new framework closer to probabilistic models and better suited for deep learning, by defining an energy function for training

\begin{definition}[Restricted Kernel Machine for Training]
\label{def:rkm-training}
Given $\bm{\phi}_i \in \mathcal{F}$ as we defined them earlier. The variables are the same linear operator as earlier $\bm{\varrho} : \mathcal{L} \rightarrow \mathcal{F}$, $\bm{h}_i \in \mathcal{L}$, $\bm{\Omega} : \mathcal{L} \rightarrow \mathcal{L}$, which is diagonal in the canonical basis of $\mathcal{E}$, \emph{i.e.}, $\bm{\Omega} = \sum_{p=1}^q\omega_p \bm{e}_p\bm{e}_p^\ast$. The energy function for training is defined as
\begin{equation}
    J_{\mathrm{T}} = \sum_{i=1}^N E_T(\bm{h}_i) + \frac12 \mathrm{tr}\left(\bm{\varrho}^\ast\bm{\varrho}\right),
\end{equation}
with $\mathrm{tr}$ representing the trace of the operator and
    \begin{equation}
\label{eq:rkm}
    E_J\left(\bm{h}_i\right) = -\bm{\phi}_i^\ast\bm{\varrho}\bm{h}_i +\frac12 \bm{h}_i^\ast\bm{\Omega}\bm{h}_i.
\end{equation}
Training the model consists in characterizing the stationary points of the energy function.
\end{definition}

When characterizing the stationary points, we obtain
\begin{eqnarray}
    \frac{\partial J_{\mathrm{T}}}{\partial \bm{h}_i} = 0 &\Longleftrightarrow& \bm{\varrho}^\ast\bm{\phi}_i = \bm{\Omega}\bm{h}_i, \quad \forall i\\
    \frac{\partial J_{\mathrm{T}}}{\partial \bm{\varrho}} = 0 &\Longleftrightarrow& \bm{\varrho} = \sum_{i=1}^N \bm{\phi}_i\bm{h}_i^\ast.
\end{eqnarray}
If we combine those two equations and express them into the canonical basis of $\mathcal{E}$, we get $\left(\bm{h}_i^\ast\bm{e}_p\right)k\left(\bm{x}_i,\bm{x}_{i'}\right) = \left(\bm{h_{i'}}^\ast\bm{e}_p\right)\omega_p$ for all $i,i' = 1,\ldots,N$ and $p=1,\ldots,q$. This leads to $\omega_p=\lambda_p$ and $\bm{h}_i = \sum_{p=1}^q \left(\bm{\psi}_p^\ast\bm{e}_i\right)\bm{e}_p^\ast$, where $\left\{\left(\lambda_p,\bm{\psi}_p\right)\right\}_{p=1}^q$ are $q$ eigenpairs of $\PaP$.

Further extensions have also allowed the model to tackle generation~\cite{schreurs, gen-rkm}.
\begin{definition}[Restricted Kernel Machines for Generation]
Given a $\bm{h} \in \mathcal{L}$ and the $\bm{\varrho}$ found by the trained model (Def.~\ref{def:rkm-training}). The energy function for the generation of $\bm{\phi} \in \mathcal{F}$ is given by
\begin{equation}
    J_{\mathrm{G}} = E_G\left(\bm{\phi}\right) = -\bm{\phi}^\ast\bm{\varrho}\bm{h} +\frac12 \bm{\phi}^\ast\bm{\phi}.
\end{equation}
The generation in itself consists in characterizing the stationary points of the energy function.
\end{definition}

Again, characterizing the stationary points gives
\begin{equation}
    \frac{\partial J_G}{\partial \bm{\phi}} = 0 \quad \Longleftrightarrow \quad \bm{\phi} = \bm{\varrho}\bm{h}.
\end{equation}

\subsection{Connections with Probabilistic PCA}
